Weakly-Supervised Image Semantic Segmentation Using Graph Convolutional Networks

This work addresses weakly-supervised image semantic segmentation based on image-level class labels. One common approach to this task is to propagate the activation scores of Class Activation Maps (CAMs) using a random-walk mechanism in order to arrive at complete pseudo labels for training a semantic segmentation network in a fully-supervised manner. However, the feed-forward nature of the random walk imposes no regularization on the quality of the resulting complete pseudo labels. To overcome this issue, we propose a Graph Convolutional Network (GCN)-based feature propagation framework. We formulate the generation of complete pseudo labels as a semi-supervised learning task and learn a 2-layer GCN separately for every training image by back-propagating a Laplacian and an entropy regularization loss. Experimental results on the PASCAL VOC 2012 dataset confirm the superiority of our scheme to several state-of-the-art baselines. Our code is available at https://github.com/Xavier-Pan/WSGCN.

==> table/exp_stage2.tex <==
\begin{figure}[b!]\label{fig_app}
    \small
    \centering
    \setlength\tabcolsep{0.01cm}
    \begin{tabular}{cccc}
        %\raisebox{1.75\normalbaselineskip}[0pt][0pt]{}\\
        %{\parbox{2cm}{\begin{center}Image \end{center}}}\\
        %{\parbox{2cm}{\begin{center}WSGCN-I \end{center}}}\\
        %\parbox{1.8cm}{\begin{center}Image}&Image&Image&Image
        %\parbox{1.8cm}{\begin{center}Image\end{center}}&\parbox{1.8cm}{\begin{center}WSGCN-I\end{center}}&\parbox{1.8cm}{\begin{center}Image\end{center}}&\parbox{1.8cm}{\begin{center}WSGCN-I\end{center}}\\
     
        \includegraphics[width=2cm,height=2.1cm]{figures/result_img/stageII/res101_ours/2008_000012.png}&
        \includegraphics[width=2cm,height=2.1cm]{figures/result_img/stageII/res101_ours/2008_000712.png}
        \includegraphics[width=2cm,height=2.1cm]{figures/result_img/stageII/res101_ours/2008_000160.png}&
        \includegraphics[width=2cm,height=2.1cm]{figures/result_img/stageII/res101_ours/2008_008631.png}
        \\
        \includegraphics[width=2cm,height=2.1cm]{figures/result_img/stageII/res101_ours/2009_002310.png}&
        \includegraphics[width=2cm,height=2.1cm]{figures/result_img/stageII/res101_ours/2010_001500.png}
        \includegraphics[width=2cm,height=2.1cm]{figures/result_img/stageII/res101_ours/2010_002358.png}&
        \includegraphics[width=2cm,height=2.1cm]{figures/result_img/stageII/res101_ours/2010_004881.png}
        \\
    \end{tabular}
    \caption{Semantic segmentation results of the proposed method on PASCAL VOC 2012 test set.}
    \label{fig_stage2}
    \vspace{-0.8em}
\end{figure}


